Whence Is A Model Fair? Fixing Fairness Bugs via Propensity Score Matching

Fairness-aware learning aims to mitigate discrimination against specific protected social groups (e.g., those categorized by gender, ethnicity, age) while minimizing predictive performance loss. Despite efforts to improve fairness in machine learning, prior studies have shown that many models remain unfair when measured against various fairness metrics. In this paper, we examine whether the way training and testing data are sampled affects the reliability of reported fairness metrics. Since training and test sets are often randomly sampled from the same population, bias present in the training data may still exist in the test data, potentially skewing fairness assessments. To address this, we propose FairMatch, a post-processing method that applies propensity score matching to evaluate and mitigate bias. FairMatch identifies control and treatment pairs with similar propensity scores in the test set and adjusts decision thresholds for different subgroups accordingly. For samples that cannot be matched, we perform probabilistic calibration using fairness-aware loss functions. Experimental results demonstrate that our approach can (a) precisely locate subsets of the test data where the model is unbiased, and (b) significantly reduce bias on the remaining data. Overall, propensity score matching offers a principled way to improve both fairness evaluation and mitigation, without sacrificing predictive performance.

==> name.tex <==
 \section{4}
 
 \subsection{Search space}
 explains why the problem cannot be optimized manually or by brute force within a reasonable timeframe
 
 
  \subsection{SConstraint}
 
 describes the search space (e.g., constraints, independent variables choices)

  \subsection{SSimpliying assumptions}
 nrbrt motr thatn size (in ptincipel that can be done e.g. by running an initial PCA or a "straw study" that jsyt explroes the most constraining assumptions first)

 @INPROCEEDINGS{6693104,
  author={Sayyad, Abdel Salam and Ingram, Joseph and Menzies, Tim and Ammar, Hany},
  booktitle={2013 28th IEEE/ACM International Conference on Automated Software Engineering (ASE)}, 
  title={Scalable product line configuration: A straw to break the camel's back}, 
  year={2013},
  volume={},
  number={},
  pages={465-474},
  doi={10.1109/ASE.2013.6693104}}
  
 
  \subsection{justifies the choice of algorithm underlying the approach}

  prior work showed that. we build on it in the following way...

   explains whether the study explores a new problem type (or a new area within an existing problem space), or how it reproduces, replicates, or improves upon prior work
   
  
\subsection{pronlem formulation}
-  a description of what a solution represents
- how it is represented
- and how it is manipulated

\subsection{fitness}
 explicitly defines all fitness functions, including the type of goals that are optimized and the equations for calculating fitness values

\subsection{soundness}
  motivates the novelty and soundness of the proposed approach15



 
 
=====================

 
 
\ssubection{data  }

add subsubsub headings

 explains in detail how subjects or datasets were collected/chosen to mitigate selection bias and improve the generalization of findings

 
 provides random data splits (e.g., those used in data-driven approaches) or ensures splits are reproducibile.
 compares distributions (rather than means) of results using appropriate statistics
 

EITHER: makes data publicly available OR: explains why this is not possible11
 identifies and explains all possible sources of stochasticity12

  describes the main features of the subjects used to run and evaluate the optimization approach(es) and discuss what characterizes the different instances in terms of "hardness"
  

   EITHER: clearly describes (and follows) a sound process to collect and prepare the datasets used to run and to evaluate the optimization approach
OR: if the subjects are taken from previous work, fully reference the original source and explain whether any transformation or cleaning was applied to the datasets


 \ssubection{experimental method}

 add subsubsub headings

  provides a replication package that conforms to SIGSOFT standards for artifacts14.

  
explicitly defines evaluated approaches, including the techniques, specific heuristics, and the parameters and their values10


 executes stochastic approaches or elements multiple times
 samples from data multiple times in a controlled manner (where appropriate and possible)
 performs multiple trials either as a cross-validation (multiple independent executions) or temporally (multiple applications as part of a timed sequence), depending on the problem at hand


  compares approaches to a justified and appropriate baseline7





 justifies the parameter values used when executing the evaluated approaches (and note that experiments trying a wide range of different parameter values would be extraordinary, see below)


 \subsection{evaluation Criteria}

 add subsubsub headings

  compares solutions using an appropriate meta-evaluation criteria16; justifies the chosen criteria
 clearly distinguishes evidence-based results from interpretations and speculation17

==> tables <==
% \begin{table*}[]
% \caption{Results for RQ4.  For all performance metrics, greater is better; for all fairness metrics, smaller is better. Here, cells marked in darker colors are better than those marked in lighter colors within the same dataset block. The ranks indicated by colors are determined by the Scott-Knott test. "LR" denotes the baseline logistic regression model.}
% \label{rq3-1}
% {\scriptsize
% %\resizebox{\textwidth}{!}{%
% \begin{center}\begin{tabular}{|c|c|cccccccc|}
% \hline
% Dataset &
%   Method &
%   \multicolumn{1}{c}{Accuracy} &
%   \multicolumn{1}{c}{Precision} &
%   \multicolumn{1}{c}{Recall} &
%   \multicolumn{1}{c}{F1} &
%   \multicolumn{1}{c}{AOD} &
%   \multicolumn{1}{c}{EOD} &
%   \multicolumn{1}{c}{SPD} &
%   \multicolumn{1}{c|}{DI} \\ \hline
% Adult: Sex &
%   LR &
%   \cellcolor[HTML]{969696}84 &
%   \cellcolor[HTML]{969696}73 &
%   \cellcolor[HTML]{EFEFEF}59 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}2 &
%   12 &
%   \cellcolor[HTML]{EFEFEF}19 &
%   74 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}84 &
%   \cellcolor[HTML]{969696}73 &
%   54 &
%   \cellcolor[HTML]{EFEFEF}62 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}12 &
%   \cellcolor[HTML]{969696}50 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}84 &
%   \cellcolor[HTML]{969696}73 &
%   56 &
%   \cellcolor[HTML]{969696}64 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}13 &
%   \cellcolor[HTML]{EFEFEF}57 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}84 &
%   \cellcolor[HTML]{969696}73 &
%   \cellcolor[HTML]{EFEFEF}59 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}18 &
%   \cellcolor[HTML]{EFEFEF}68 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}84 &
%   \cellcolor[HTML]{EFEFEF}65 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}65 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{EFEFEF}9 &
%   \cellcolor[HTML]{969696}14 &
%   \cellcolor[HTML]{969696}52 \\ \hline
% Adult: Race &
%   LR &
%   \cellcolor[HTML]{969696}85 &
%   \cellcolor[HTML]{969696}74 &
%   \cellcolor[HTML]{969696}59 &
%   \cellcolor[HTML]{969696}66 &
%   4 &
%   13 &
%   11 &
%   52 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}84 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{969696}59 &
%   \cellcolor[HTML]{969696}65 &
%   \cellcolor[HTML]{EFEFEF}2 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}7 &
%   \cellcolor[HTML]{969696}33 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}85 &
%   \cellcolor[HTML]{969696}73 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{EFEFEF}2 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}9 &
%   \cellcolor[HTML]{EFEFEF}41 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}85 &
%   \cellcolor[HTML]{969696}73 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{EFEFEF}2 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   \cellcolor[HTML]{EFEFEF}9 &
%   \cellcolor[HTML]{EFEFEF}44 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}85 &
%   \cellcolor[HTML]{969696}73 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}1 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}7 &
%   \cellcolor[HTML]{969696}28 \\ \hline
% Compas: Sex &
%   LR &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{EFEFEF}74 &
%   \cellcolor[HTML]{969696}70 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   24 &
%   33 &
%   37 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}65 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{EFEFEF}76 &
%   \cellcolor[HTML]{969696}70 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}6 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{EFEFEF}76 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}15 &
%   \cellcolor[HTML]{EFEFEF}20 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{EFEFEF}75 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{EFEFEF}12 &
%   \cellcolor[HTML]{EFEFEF}18 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}65 &
%   \cellcolor[HTML]{EFEFEF}64 &
%   \cellcolor[HTML]{969696}82 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{EFEFEF}14 &
%   \cellcolor[HTML]{EFEFEF}17 \\ \hline
% Compas: Race &
%   LR &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{EFEFEF}74 &
%   \cellcolor[HTML]{969696}70 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   11 &
%   20 &
%   27 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}65 &
%   \cellcolor[HTML]{EFEFEF}78 &
%   \cellcolor[HTML]{969696}70 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{EFEFEF}8 &
%   \cellcolor[HTML]{EFEFEF}11 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{EFEFEF}76 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   \cellcolor[HTML]{EFEFEF}9 &
%   \cellcolor[HTML]{FFFFFF}16 &
%   \cellcolor[HTML]{FFFFFF}23 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{EFEFEF}75 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   \cellcolor[HTML]{FFFFFF}15 &
%   \cellcolor[HTML]{FFFFFF}21 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}65 &
%   \cellcolor[HTML]{EFEFEF}64 &
%   \cellcolor[HTML]{969696}81 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}5 \\ \hline
% Bank: Age &
%   LR &
%   \cellcolor[HTML]{969696}90 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}40 &
%   \cellcolor[HTML]{969696}50 &
%   6 &
%   17 &
%   11 &
%   151 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}90 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}40 &
%   \cellcolor[HTML]{969696}50 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}68 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}90 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}39 &
%   \cellcolor[HTML]{969696}50 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}7 &
%   \cellcolor[HTML]{969696}7 &
%   \cellcolor[HTML]{969696}91 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}90 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}40 &
%   \cellcolor[HTML]{969696}50 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{EFEFEF}14 &
%   \cellcolor[HTML]{EFEFEF}9 &
%   \cellcolor[HTML]{EFEFEF}130 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}90 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}40 &
%   \cellcolor[HTML]{969696}50 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{EFEFEF}14 &
%   \cellcolor[HTML]{EFEFEF}9 &
%   \cellcolor[HTML]{EFEFEF}128 \\ \hline
% German: Sex &
%   LR &
%   \cellcolor[HTML]{969696}77 &
%   \cellcolor[HTML]{EFEFEF}80 &
%   \cellcolor[HTML]{969696}88 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{EFEFEF}7 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   \cellcolor[HTML]{EFEFEF}12 &
%   \cellcolor[HTML]{EFEFEF}15 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{EFEFEF}79 &
%   \cellcolor[HTML]{969696}87 &
%   \cellcolor[HTML]{969696}82 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}6 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{EFEFEF}78 &
%   \cellcolor[HTML]{969696}89 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}6 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{EFEFEF}80 &
%   \cellcolor[HTML]{969696}87 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}6 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{EFEFEF}78 &
%   \cellcolor[HTML]{969696}81 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}6 \\ \hline
% Health: Age &
%   LR &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}80 &
%   \cellcolor[HTML]{969696}84 &
%   \cellcolor[HTML]{969696}82 &
%   11 &
%   12 &
%   41 &
%   60 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}80 &
%   \cellcolor[HTML]{969696}81 &
%   \cellcolor[HTML]{969696}81 &
%   10 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{969696}24 &
%   \cellcolor[HTML]{969696}43 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}80 &
%   \cellcolor[HTML]{969696}81 &
%   \cellcolor[HTML]{969696}81 &
%   11 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{969696}23 &
%   \cellcolor[HTML]{969696}43 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}82 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}82 &
%   \cellcolor[HTML]{EFEFEF}7 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{969696}23 &
%   \cellcolor[HTML]{EFEFEF}50 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}81 &
%   \cellcolor[HTML]{969696}81 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}81 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}25 &
%   \cellcolor[HTML]{969696}44 \\ \hline
% MEPS: Race &
%   LR &
%   \cellcolor[HTML]{969696}87 &
%   \cellcolor[HTML]{969696}71 &
%   42 &
%   \cellcolor[HTML]{969696}53 &
%   \cellcolor[HTML]{EFEFEF}8 &
%   23 &
%   14 &
%   68 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{EFEFEF}67 &
%   35 &
%   \cellcolor[HTML]{EFEFEF}46 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{EFEFEF}37 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{EFEFEF}70 &
%   38 &
%   \cellcolor[HTML]{EFEFEF}49 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}15 &
%   \cellcolor[HTML]{969696}9 &
%   62 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}87 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{EFEFEF}40 &
%   \cellcolor[HTML]{969696}51 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}9 &
%   57 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}88 &
%   53 &
%   \cellcolor[HTML]{969696}53 &
%   \cellcolor[HTML]{969696}53 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}20 \\ \hline
% \end{tabular}
% \end{center}}
% \end{table*}


% \begin{table*}[]
% \caption{More Results for RQ4.  For all performance metrics, greater is better; for all fairness metrics, smaller is better. Here, cells marked in darker colors are better than those marked in lighter colors within the same dataset block. "XGB" denotes the baseline gradient boosting model.}
% \label{rq3-2}
% \scriptsize
% \centering\begin{tabular}{|c|c|cccccccc|}
% \hline
% Dataset &
%   Method &
%   \multicolumn{1}{c}{Accuracy} &
%   \multicolumn{1}{c}{Precision} &
%   \multicolumn{1}{c}{Recall} &
%   \multicolumn{1}{c}{F1} &
%   \multicolumn{1}{c}{AOD} &
%   \multicolumn{1}{c}{EOD} &
%   \multicolumn{1}{c}{SPD} &
%   \multicolumn{1}{c|}{DI} \\ \hline
% Adult: Sex &
%   XGB &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   10 &
%   17 &
%   72 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}85 &
%   \cellcolor[HTML]{969696}77 &
%   \cellcolor[HTML]{EFEFEF}57 &
%   \cellcolor[HTML]{EFEFEF}66 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}12 &
%   \cellcolor[HTML]{969696}50 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}59 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}1 &
%   8 &
%   16 &
%   69 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}61 &
%   \cellcolor[HTML]{969696}69 &
%   \cellcolor[HTML]{969696}2 &
%   8 &
%   17 &
%   65 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}77 &
%   \cellcolor[HTML]{969696}61 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}1 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   \cellcolor[HTML]{EFEFEF}14 &
%   \cellcolor[HTML]{EFEFEF}60 \\ \hline
% Adult: Race &
%   XGB &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{EFEFEF}2 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{EFEFEF}8 &
%   40 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}85 &
%   \cellcolor[HTML]{EFEFEF}73 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{EFEFEF}65 &
%   \cellcolor[HTML]{969696}1 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}31 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{EFEFEF}2 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{EFEFEF}8 &
%   \cellcolor[HTML]{EFEFEF}37 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}1 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{EFEFEF}8 &
%   39 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}61 &
%   \cellcolor[HTML]{969696}69 &
%   \cellcolor[HTML]{969696}1 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}7 &
%   \cellcolor[HTML]{EFEFEF}37 \\ \hline
% Compas: Sex &
%   XGB &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}77 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   10 &
%   17 &
%   25 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}8 &
%   \cellcolor[HTML]{969696}11 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}69 &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{EFEFEF}8 &
%   \cellcolor[HTML]{EFEFEF}15 &
%   \cellcolor[HTML]{EFEFEF}21 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{EFEFEF}9 &
%   \cellcolor[HTML]{EFEFEF}14 &
%   \cellcolor[HTML]{EFEFEF}21 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}74 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}9 &
%   \cellcolor[HTML]{969696}13 \\ \hline
% Compas: Race &
%   XGB &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}77 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{EFEFEF}12 &
%   18 &
%   25 \\
%  &
%   EGR &
%   \cellcolor[HTML]{EFEFEF}66 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{969696}71 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}5 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}69 &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{EFEFEF}11 &
%   17 &
%   25 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}14 &
%   21 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}68 &
%   \cellcolor[HTML]{969696}69 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{969696}72 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}9 &
%   \cellcolor[HTML]{EFEFEF}13 \\ \hline
% Bank: Age &
%   XBG &
%   \cellcolor[HTML]{969696}91 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}55 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}11 &
%   105 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}91 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}53 &
%   \cellcolor[HTML]{969696}59 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}7 &
%   \cellcolor[HTML]{969696}8 &
%   \cellcolor[HTML]{969696}78 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}91 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}55 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}9 &
%   \cellcolor[HTML]{EFEFEF}93 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}91 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{969696}55 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}8 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}99 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}91 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{969696}55 &
%   \cellcolor[HTML]{969696}60 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}8 &
%   \cellcolor[HTML]{969696}80 \\ \hline
% German: Sex &
%   XGB &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}88 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{EFEFEF}5 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}88 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   7 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}88 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{EFEFEF}4 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{EFEFEF}5 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}88 &
%   \cellcolor[HTML]{969696}83 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}3 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}87 &
%   \cellcolor[HTML]{969696}82 &
%   \cellcolor[HTML]{969696}2 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}4 \\ \hline
% Health: Age &
%   XGB &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{969696}6 &
%   16 &
%   \cellcolor[HTML]{EFEFEF}30 &
%   50 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{EFEFEF}11 &
%   \cellcolor[HTML]{EFEFEF}11 &
%   \cellcolor[HTML]{969696}26 &
%   \cellcolor[HTML]{EFEFEF}46 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}75 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{EFEFEF}11 &
%   \cellcolor[HTML]{969696}9 &
%   \cellcolor[HTML]{969696}26 &
%   \cellcolor[HTML]{EFEFEF}44 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}77 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}9 &
%   \cellcolor[HTML]{969696}25 &
%   \cellcolor[HTML]{EFEFEF}45 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}79 &
%   \cellcolor[HTML]{969696}78 &
%   \cellcolor[HTML]{969696}76 &
%   \cellcolor[HTML]{969696}77 &
%   \cellcolor[HTML]{969696}9 &
%   14 &
%   \cellcolor[HTML]{969696}24 &
%   \cellcolor[HTML]{969696}41 \\ \hline
% MEPS: Race &
%   XGB &
%   \cellcolor[HTML]{969696}87 &
%   \cellcolor[HTML]{969696}65 &
%   \cellcolor[HTML]{EFEFEF}42 &
%   \cellcolor[HTML]{969696}51 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   15 &
%   12 &
%   63 \\
%  &
%   EGR &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}68 &
%   36 &
%   \cellcolor[HTML]{EFEFEF}47 &
%   \cellcolor[HTML]{969696}3 &
%   \cellcolor[HTML]{969696}6 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}39 \\
%  &
%   FAXAI &
%   \cellcolor[HTML]{969696}87 &
%   \cellcolor[HTML]{969696}67 &
%   \cellcolor[HTML]{EFEFEF}41 &
%   \cellcolor[HTML]{969696}51 &
%   \cellcolor[HTML]{EFEFEF}6 &
%   \cellcolor[HTML]{EFEFEF}15 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}60 \\
%  &
%   FairMask &
%   \cellcolor[HTML]{969696}86 &
%   \cellcolor[HTML]{969696}66 &
%   \cellcolor[HTML]{EFEFEF}42 &
%   \cellcolor[HTML]{969696}52 &
%   \cellcolor[HTML]{EFEFEF}5 &
%   \cellcolor[HTML]{EFEFEF}8 &
%   \cellcolor[HTML]{EFEFEF}10 &
%   \cellcolor[HTML]{EFEFEF}56 \\
%  &
%   {\bf FairMatch} &
%   \cellcolor[HTML]{969696}85 &
%   \cellcolor[HTML]{EFEFEF}53 &
%   \cellcolor[HTML]{969696}50 &
%   \cellcolor[HTML]{969696}51 &
%   \cellcolor[HTML]{969696}4 &
%   \cellcolor[HTML]{969696}5 &
%   \cellcolor[HTML]{969696}7 &
%   \cellcolor[HTML]{969696}38 \\ \hline
% \end{tabular}%
% \end{table*}



2024-05-20

\begin{tabular}{|c|ccccc|ccccc|ccccc|ccccc}
\hline
Dataset &
  \multicolumn{5}{c|}{Adult: Sex} &
  \multicolumn{5}{c|}{Adult: Race} &
  \multicolumn{5}{c|}{Compas: Sex} &
  \multicolumn{5}{c|}{Compas: Race} \\ \hline
Method &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \multicolumn{1}{c|}{\textbf{FairMatch}} \\ \hline
Accuracy &
  \cellcolor[HTML]{969696}84 &
  \cellcolor[HTML]{969696}84 &
  \cellcolor[HTML]{969696}84 &
  \cellcolor[HTML]{969696}84 &
  \cellcolor[HTML]{969696}84 &
  \cellcolor[HTML]{969696}85 &
  \cellcolor[HTML]{969696}84 &
  \cellcolor[HTML]{969696}85 &
  \cellcolor[HTML]{969696}85 &
  \cellcolor[HTML]{969696}85 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}65 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}65 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}66 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}65} \\
Precision &
  \cellcolor[HTML]{969696}73 &
  \cellcolor[HTML]{969696}73 &
  \cellcolor[HTML]{969696}73 &
  \cellcolor[HTML]{969696}73 &
  \cellcolor[HTML]{BBBBBB}65 &
  \cellcolor[HTML]{969696}74 &
  \cellcolor[HTML]{969696}72 &
  \cellcolor[HTML]{969696}73 &
  \cellcolor[HTML]{969696}73 &
  \cellcolor[HTML]{969696}73 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{BBBBBB}64 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}65 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BBBBBB}64} \\
Recall &
  \cellcolor[HTML]{BBBBBB}59 &
  54 &
  56 &
  \cellcolor[HTML]{BBBBBB}59 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}59 &
  \cellcolor[HTML]{969696}59 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{BBBBBB}74 &
  \cellcolor[HTML]{BBBBBB}76 &
  \cellcolor[HTML]{BBBBBB}76 &
  \cellcolor[HTML]{BBBBBB}75 &
  \cellcolor[HTML]{969696}82 &
  \cellcolor[HTML]{BBBBBB}74 &
  \cellcolor[HTML]{BBBBBB}78 &
  \cellcolor[HTML]{BBBBBB}76 &
  \cellcolor[HTML]{BBBBBB}75 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}81} \\
F1 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{BBBBBB}62 &
  \cellcolor[HTML]{969696}64 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}65 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}65 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}70 &
  \cellcolor[HTML]{969696}70 &
  \cellcolor[HTML]{969696}71 &
  \cellcolor[HTML]{969696}71 &
  \cellcolor[HTML]{969696}72 &
  \cellcolor[HTML]{969696}70 &
  \cellcolor[HTML]{969696}70 &
  \cellcolor[HTML]{969696}71 &
  \cellcolor[HTML]{969696}71 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}71} \\
AOD &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}2 &
  4 &
  \cellcolor[HTML]{BBBBBB}2 &
  \cellcolor[HTML]{BBBBBB}2 &
  \cellcolor[HTML]{BBBBBB}2 &
  \cellcolor[HTML]{969696}1 &
  \cellcolor[HTML]{BBBBBB}6 &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{BBBBBB}6 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}6 &
  \cellcolor[HTML]{969696}3 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}4} \\
EOD &
  12 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{BBBBBB}10 &
  \cellcolor[HTML]{BBBBBB}9 &
  13 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{BBBBBB}6 &
  \cellcolor[HTML]{969696}4 &
  24 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{BBBBBB}10 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{969696}6 &
  11 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{BBBBBB}9 &
  \cellcolor[HTML]{BBBBBB}6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}4} \\
SPD &
  \cellcolor[HTML]{BBBBBB}19 &
  \cellcolor[HTML]{969696}12 &
  \cellcolor[HTML]{969696}13 &
  \cellcolor[HTML]{BBBBBB}18 &
  \cellcolor[HTML]{969696}14 &
  11 &
  \cellcolor[HTML]{969696}7 &
  \cellcolor[HTML]{969696}9 &
  \cellcolor[HTML]{BBBBBB}9 &
  \cellcolor[HTML]{969696}7 &
  33 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{BBBBBB}15 &
  \cellcolor[HTML]{BBBBBB}12 &
  \cellcolor[HTML]{BBBBBB}14 &
  20 &
  \cellcolor[HTML]{BBBBBB}8 &
  \cellcolor[HTML]{FFFFFF}16 &
  \cellcolor[HTML]{FFFFFF}15 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}3} \\
DI &
  74 &
  \cellcolor[HTML]{969696}50 &
  \cellcolor[HTML]{BBBBBB}57 &
  \cellcolor[HTML]{BBBBBB}68 &
  \cellcolor[HTML]{969696}52 &
  52 &
  \cellcolor[HTML]{969696}33 &
  \cellcolor[HTML]{BBBBBB}41 &
  \cellcolor[HTML]{BBBBBB}44 &
  \cellcolor[HTML]{969696}28 &
  37 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{BBBBBB}20 &
  \cellcolor[HTML]{BBBBBB}18 &
  \cellcolor[HTML]{BBBBBB}17 &
  27 &
  \cellcolor[HTML]{BBBBBB}11 &
  \cellcolor[HTML]{FFFFFF}23 &
  \cellcolor[HTML]{FFFFFF}21 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}5} \\ \hline
Dataset &
  \multicolumn{5}{c|}{Bank: Age} &
  \multicolumn{5}{c|}{German: Sex} &
  \multicolumn{5}{c|}{Health: Age} &
  \multicolumn{5}{c|}{MEPS: Race} \\ \hline
Method &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  LR &
  EGR &
  FAXAI &
  FairMask &
  \multicolumn{1}{c|}{\textbf{FairMatch}} \\ \hline
Accuracy &
  \cellcolor[HTML]{969696}90 &
  \cellcolor[HTML]{969696}90 &
  \cellcolor[HTML]{969696}90 &
  \cellcolor[HTML]{969696}90 &
  \cellcolor[HTML]{969696}90 &
  \cellcolor[HTML]{969696}77 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}76 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}87 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}87 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}88} \\
Precision &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{BBBBBB}80 &
  \cellcolor[HTML]{BBBBBB}79 &
  \cellcolor[HTML]{BBBBBB}78 &
  \cellcolor[HTML]{BBBBBB}80 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}80 &
  \cellcolor[HTML]{969696}80 &
  \cellcolor[HTML]{969696}80 &
  \cellcolor[HTML]{969696}82 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}71 &
  \cellcolor[HTML]{BBBBBB}67 &
  \cellcolor[HTML]{969696}70 &
  \cellcolor[HTML]{969696}71 &
  \multicolumn{1}{c|}{53} \\
Recall &
  \cellcolor[HTML]{969696}40 &
  \cellcolor[HTML]{969696}40 &
  \cellcolor[HTML]{969696}39 &
  \cellcolor[HTML]{969696}40 &
  \cellcolor[HTML]{969696}40 &
  \cellcolor[HTML]{969696}88 &
  \cellcolor[HTML]{969696}87 &
  \cellcolor[HTML]{969696}89 &
  \cellcolor[HTML]{969696}87 &
  \cellcolor[HTML]{BBBBBB}78 &
  \cellcolor[HTML]{969696}84 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}79 &
  42 &
  35 &
  38 &
  \cellcolor[HTML]{BBBBBB}40 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}53} \\
F1 &
  \cellcolor[HTML]{969696}50 &
  \cellcolor[HTML]{969696}50 &
  \cellcolor[HTML]{969696}50 &
  \cellcolor[HTML]{969696}50 &
  \cellcolor[HTML]{969696}50 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}82 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}82 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}82 &
  \cellcolor[HTML]{969696}81 &
  \cellcolor[HTML]{969696}53 &
  \cellcolor[HTML]{BBBBBB}46 &
  \cellcolor[HTML]{BBBBBB}49 &
  \cellcolor[HTML]{969696}51 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}53} \\
AOD &
  6 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{BBBBBB}7 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}4 &
  11 &
  10 &
  11 &
  \cellcolor[HTML]{BBBBBB}7 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}8 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{969696}4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}4} \\
EOD &
  17 &
  \cellcolor[HTML]{969696}5 &
  \cellcolor[HTML]{969696}7 &
  \cellcolor[HTML]{BBBBBB}14 &
  \cellcolor[HTML]{BBBBBB}14 &
  \cellcolor[HTML]{BBBBBB}6 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{969696}3 &
  12 &
  \cellcolor[HTML]{BBBBBB}10 &
  \cellcolor[HTML]{BBBBBB}10 &
  \cellcolor[HTML]{BBBBBB}10 &
  \cellcolor[HTML]{969696}6 &
  23 &
  \cellcolor[HTML]{969696}5 &
  \cellcolor[HTML]{969696}15 &
  \cellcolor[HTML]{BBBBBB}10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}4} \\
SPD &
  11 &
  \cellcolor[HTML]{969696}5 &
  \cellcolor[HTML]{969696}7 &
  \cellcolor[HTML]{BBBBBB}9 &
  \cellcolor[HTML]{BBBBBB}9 &
  \cellcolor[HTML]{BBBBBB}12 &
  \cellcolor[HTML]{969696}5 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}5 &
  \cellcolor[HTML]{969696}4 &
  41 &
  \cellcolor[HTML]{969696}24 &
  \cellcolor[HTML]{969696}23 &
  \cellcolor[HTML]{969696}23 &
  \cellcolor[HTML]{969696}25 &
  14 &
  \cellcolor[HTML]{969696}5 &
  \cellcolor[HTML]{969696}9 &
  \cellcolor[HTML]{BBBBBB}9 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}4} \\
DI &
  151 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}91 &
  \cellcolor[HTML]{BBBBBB}130 &
  \cellcolor[HTML]{BBBBBB}128 &
  \cellcolor[HTML]{BBBBBB}15 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{969696}6 &
  60 &
  \cellcolor[HTML]{969696}43 &
  \cellcolor[HTML]{969696}43 &
  \cellcolor[HTML]{BBBBBB}50 &
  \cellcolor[HTML]{969696}44 &
  68 &
  \cellcolor[HTML]{BBBBBB}37 &
  62 &
  57 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}20} \\ \hline
\end{tabular}



\begin{tabular}{|c|ccccc|ccccc|cccccccccc}
\hline
Dataset &
  \multicolumn{5}{c|}{Adult: Sex} &
  \multicolumn{5}{c|}{Adult: Race} &
  \multicolumn{5}{c|}{Compass: Sex} &
  \multicolumn{5}{c|}{Compass: Race} \\ \hline
Method &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \multicolumn{1}{c|}{\textbf{FairMatch}} &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \multicolumn{1}{c|}{\textbf{FairMatch}} \\ \hline
Accuracy &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}85 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}85 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}68 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}67} &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}68 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}68} \\
Precision &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}77 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}77 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{BBBBBB}73 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}69 &
  \cellcolor[HTML]{969696}68 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}68} &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}69 &
  \cellcolor[HTML]{969696}68 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}69} \\
Recall &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{BBBBBB}57 &
  \cellcolor[HTML]{969696}59 &
  \cellcolor[HTML]{969696}61 &
  \cellcolor[HTML]{969696}61 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}61 &
  \cellcolor[HTML]{969696}77 &
  \cellcolor[HTML]{969696}76 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}75 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}74} &
  \cellcolor[HTML]{969696}77 &
  \cellcolor[HTML]{969696}76 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}76 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}76} \\
F1 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{BBBBBB}66 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}69 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{BBBBBB}65 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}69 &
  \cellcolor[HTML]{969696}72 &
  \cellcolor[HTML]{969696}71 &
  \cellcolor[HTML]{969696}72 &
  \cellcolor[HTML]{969696}72 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}71} &
  \cellcolor[HTML]{969696}72 &
  \cellcolor[HTML]{969696}71 &
  \cellcolor[HTML]{969696}72 &
  \cellcolor[HTML]{969696}72 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}72} \\
AOD &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}1 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}1 &
  \cellcolor[HTML]{BBBBBB}2 &
  \cellcolor[HTML]{969696}1 &
  \cellcolor[HTML]{BBBBBB}2 &
  \cellcolor[HTML]{969696}1 &
  \cellcolor[HTML]{969696}1 &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}2 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}3} &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{969696}2 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}3} \\
EOD &
  10 &
  \cellcolor[HTML]{969696}2 &
  8 &
  8 &
  \cellcolor[HTML]{BBBBBB}6 &
  5 &
  \cellcolor[HTML]{BBBBBB}3 &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}2 &
  10 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{F3F3F3}8 &
  \cellcolor[HTML]{F3F3F3}9 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}5} &
  12 &
  \cellcolor[HTML]{969696}3 &
  11 &
  \cellcolor[HTML]{BBBBBB}10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}4} \\
SPD &
  17 &
  \cellcolor[HTML]{969696}12 &
  16 &
  17 &
  \cellcolor[HTML]{969696}14 &
  \cellcolor[HTML]{BBBBBB}8 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{BBBBBB}8 &
  \cellcolor[HTML]{BBBBBB}8 &
  \cellcolor[HTML]{969696}7 &
  17 &
  \cellcolor[HTML]{969696}8 &
  \cellcolor[HTML]{BBBBBB}15 &
  \cellcolor[HTML]{BBBBBB}14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}9} &
  18 &
  \cellcolor[HTML]{969696}4 &
  17 &
  \cellcolor[HTML]{BBBBBB}14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}9} \\
DI &
  72 &
  \cellcolor[HTML]{969696}50 &
  69 &
  65 &
  \cellcolor[HTML]{BBBBBB}60 &
  40 &
  \cellcolor[HTML]{969696}31 &
  \cellcolor[HTML]{BBBBBB}37 &
  39 &
  \cellcolor[HTML]{BBBBBB}37 &
  25 &
  \cellcolor[HTML]{969696}11 &
  \cellcolor[HTML]{BBBBBB}21 &
  \cellcolor[HTML]{BBBBBB}21 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}13} &
  25 &
  \cellcolor[HTML]{969696}5 &
  25 &
  \cellcolor[HTML]{BBBBBB}21 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}13} \\ \hline
Dataset &
  \multicolumn{5}{c|}{Bank: Age} &
  \multicolumn{5}{c|}{German: Sex} &
  \multicolumn{5}{c|}{Health: Age} &
  \multicolumn{5}{c|}{MEPS: Race} \\ \hline
Method &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \textbf{FairMatch} &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \multicolumn{1}{c|}{\textbf{FairMatch}} &
  XGB &
  EGR &
  FAXAI &
  FairMask &
  \multicolumn{1}{c|}{\textbf{FairMatch}} \\ \hline
Accuracy &
  \cellcolor[HTML]{969696}91 &
  \cellcolor[HTML]{969696}91 &
  \cellcolor[HTML]{969696}91 &
  \cellcolor[HTML]{969696}91 &
  \cellcolor[HTML]{969696}91 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}78 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}79} &
  \cellcolor[HTML]{969696}87 &
  \cellcolor[HTML]{969696}86 &
  \cellcolor[HTML]{969696}87 &
  \cellcolor[HTML]{969696}86 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}85} \\
Precision &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}66 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}79 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{969696}79 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}78} &
  \cellcolor[HTML]{969696}65 &
  \cellcolor[HTML]{969696}68 &
  \cellcolor[HTML]{969696}67 &
  \cellcolor[HTML]{969696}66 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BBBBBB}53} \\
Recall &
  \cellcolor[HTML]{969696}55 &
  \cellcolor[HTML]{969696}53 &
  \cellcolor[HTML]{969696}55 &
  \cellcolor[HTML]{969696}55 &
  \cellcolor[HTML]{969696}55 &
  \cellcolor[HTML]{969696}88 &
  \cellcolor[HTML]{969696}88 &
  \cellcolor[HTML]{969696}88 &
  \cellcolor[HTML]{969696}88 &
  \cellcolor[HTML]{969696}87 &
  \cellcolor[HTML]{969696}76 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}75 &
  \cellcolor[HTML]{969696}77 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}76} &
  \cellcolor[HTML]{BBBBBB}42 &
  36 &
  \cellcolor[HTML]{BBBBBB}41 &
  \cellcolor[HTML]{BBBBBB}42 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}50} \\
F1 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}59 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}60 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}83 &
  \cellcolor[HTML]{969696}82 &
  \cellcolor[HTML]{969696}76 &
  \cellcolor[HTML]{969696}76 &
  \cellcolor[HTML]{969696}76 &
  \cellcolor[HTML]{969696}78 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}77} &
  \cellcolor[HTML]{969696}51 &
  \cellcolor[HTML]{BBBBBB}47 &
  \cellcolor[HTML]{969696}51 &
  \cellcolor[HTML]{969696}52 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}51} \\
AOD &
  \cellcolor[HTML]{BBBBBB}4 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}6 &
  11 &
  11 &
  \cellcolor[HTML]{969696}6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BBBBBB}9} &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}6 &
  \cellcolor[HTML]{BBBBBB}5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}4} \\
EOD &
  10 &
  \cellcolor[HTML]{BBBBBB}7 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{BBBBBB}8 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}4 &
  16 &
  \cellcolor[HTML]{BBBBBB}11 &
  \cellcolor[HTML]{969696}9 &
  \cellcolor[HTML]{969696}9 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BBBBBB}14} &
  \cellcolor[HTML]{BBBBBB}15 &
  \cellcolor[HTML]{969696}6 &
  \cellcolor[HTML]{BBBBBB}15 &
  \cellcolor[HTML]{969696}8 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}5} \\
SPD &
  11 &
  \cellcolor[HTML]{969696}8 &
  \cellcolor[HTML]{BBBBBB}9 &
  \cellcolor[HTML]{BBBBBB}10 &
  \cellcolor[HTML]{969696}8 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{BBBBBB}6 &
  \cellcolor[HTML]{969696}4 &
  \cellcolor[HTML]{969696}2 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{BBBBBB}30 &
  \cellcolor[HTML]{969696}26 &
  \cellcolor[HTML]{969696}26 &
  \cellcolor[HTML]{969696}25 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}24} &
  12 &
  \cellcolor[HTML]{969696}5 &
  \cellcolor[HTML]{BBBBBB}10 &
  \cellcolor[HTML]{BBBBBB}10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}7} \\
DI &
  105 &
  \cellcolor[HTML]{969696}78 &
  \cellcolor[HTML]{BBBBBB}93 &
  \cellcolor[HTML]{BBBBBB}99 &
  \cellcolor[HTML]{969696}80 &
  \cellcolor[HTML]{BBBBBB}5 &
  7 &
  \cellcolor[HTML]{BBBBBB}5 &
  \cellcolor[HTML]{969696}3 &
  \cellcolor[HTML]{969696}4 &
  50 &
  \cellcolor[HTML]{BBBBBB}46 &
  \cellcolor[HTML]{BBBBBB}44 &
  \cellcolor[HTML]{BBBBBB}45 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}41} &
  63 &
  \cellcolor[HTML]{969696}39 &
  60 &
  \cellcolor[HTML]{BBBBBB}56 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{969696}38} \\ \hline
\end{tabular}




\begin{table*}[]
\centering
\small
\caption{The performance and fairness scores measured from testing samples. The test set is split into two subsets depending on whether they can be pair-matched via propensity scores. The ratio column shows, in percentage, the portion of each subset. Note that the SPD and DI scores for the Bank dataset are N/A since the unmatched set is extremely imbalanced and usually only contains one protected attribute.}
\begin{tabular}{|l|l|l|l|cccc|cccc|}
\hline
Dataset & Subset      & Size  & Ratio & Accuracy & Precision & Recall & F1 & AOD & EOD & SPD & DI \\ \hline
Adult: Sex                   & all         & 14653 & 1     & 85  &\cellcolor[HTML]{969696} 74        & 59     & 66 & 4  & 12  & 18  & 80 \\
                             & matched     & 2790  & 0.19  & \cellcolor[HTML]{969696}91  &\cellcolor[HTML]{969696} 74        & 50     & 59 &\cellcolor[HTML]{969696} 2   &\cellcolor[HTML]{969696} 3  &\cellcolor[HTML]{969696} 0   &\cellcolor[HTML]{969696} 0  \\
                             & non-matched & 11863 & 0.81  & 76  & 64        &\cellcolor[HTML]{969696} 63     &\cellcolor[HTML]{969696} 68 & 16   & 50   & 36  & 99 \\ \hline
Adult: Race                  & all         & 14653 & 1     & 85  &\cellcolor[HTML]{969696} 74        & 59     & 66 & 5   & 14  & 11  & 52 \\
                             & matched     & 2790  & 0.19  &\cellcolor[HTML]{969696} 89  & 71        & 48     & 57 &\cellcolor[HTML]{969696} 0   &\cellcolor[HTML]{969696} 1   &\cellcolor[HTML]{969696} 0   &\cellcolor[HTML]{969696} 0  \\
                             & non-matched & 11863 & 0.81  & 83  &\cellcolor[HTML]{969696} 74        & \cellcolor[HTML]{969696} 62     &\cellcolor[HTML]{969696} 68 & 27  & 62  & 23   & 98 \\ \hline
Compas: Sex                  & all         & 2164  & 1     & 67  & 67        & 77     & 72 & 4   & 18  & 24  & 29 \\
                             & matched     & 654   & 0.3   &\cellcolor[HTML]{969696} 70  &\cellcolor[HTML]{969696} 71        &\cellcolor[HTML]{969696} 90     &\cellcolor[HTML]{969696} 80 &\cellcolor[HTML]{969696} 3   &\cellcolor[HTML]{969696} 1   &\cellcolor[HTML]{969696} 0   &\cellcolor[HTML]{969696} 0  \\
                             & non-matched & 1510  & 0.7   & 65  & 64        & 67     & 66 & 15   & 33   & 48  & 48 \\ \hline
Compas: Race                 & all         & 2164  & 1     &\cellcolor[HTML]{969696} 66  & 67        & 74     & 70 & 6   & 11  & 20  & 27 \\
                             & matched     & 654   & 0.3   &\cellcolor[HTML]{969696} 66  &\cellcolor[HTML]{969696} 69        &\cellcolor[HTML]{969696} 80     &\cellcolor[HTML]{969696} 73 &\cellcolor[HTML]{969696} 5   & \cellcolor[HTML]{969696} 4   & \cellcolor[HTML]{969696} 0   & \cellcolor[HTML]{969696} 0  \\
                             & non-matched & 1510  & 0.7   &\cellcolor[HTML]{969696} 66  & 65        & 65     & 65 & 14   & 43   & 58   & 58  \\ \hline
Bank: Age                  & all         & 9147   & 1   & \cellcolor[HTML]{969696} 90  & \cellcolor[HTML]{969696} 66        & 41     & 51 & 8   & 22  & 12  & 162 \\
                             & matched     & 556    & 0.06    & 84 & 62        & \cellcolor[HTML]{969696} 57     &  \cellcolor[HTML]{969696} 59   &\cellcolor[HTML]{969696} 5   &\cellcolor[HTML]{969696} 1   &\cellcolor[HTML]{969696} 0   &\cellcolor[HTML]{969696} 0  \\
                             & non-matched & 8591   & 0.94   &\cellcolor[HTML]{969696} 91  & \cellcolor[HTML]{969696} 66        & 39    & 49 & 18   & 49   & N/A   & N/A  \\ \hline
German: Sex                  & all         & 300   & 1   & \cellcolor[HTML]{969696} 79  & 81        & 92     & 86 & 8   & 9  & 15  & 18 \\
                             & matched     & 56    & 0.19    &\cellcolor[HTML]{969696} 79  &\cellcolor[HTML]{969696} 83        & \cellcolor[HTML]{969696}87     & 85 &\cellcolor[HTML]{969696} 4   &\cellcolor[HTML]{969696} 3   &\cellcolor[HTML]{969696} 0   &\cellcolor[HTML]{969696} 0  \\
                             & non-matched & 244   & 0.81   &\cellcolor[HTML]{969696} 79  & 79        & 97    & \cellcolor[HTML]{969696} 88 & 4   & 66   & 59   & 64  \\ \hline
MEPS: Race                   & all         & 1461  & 1     & 87  & 71        & 43     & 53 & 15   & 33   & 14   & 74 \\
                             & matched     & 906   & 0.62  & 85  & 67        & 35     & 46 &\cellcolor[HTML]{969696} 5   &\cellcolor[HTML]{969696} 9   &\cellcolor[HTML]{969696} 0   &\cellcolor[HTML]{969696} 0  \\
                             & non-matched & 555   & 0.38  & \cellcolor[HTML]{969696} 91  & \cellcolor[HTML]{969696}78        &\cellcolor[HTML]{969696} 54     &\cellcolor[HTML]{969696} 64 & 25  & 75  & 56   & 99 \\ \hline
Heart: Age                   & all         & 89    & 1     & 80  & 76        & 80     & 78 & 8   & 29  & 29  & 48 \\
                             & matched     & 50    & 0.56  & 77  & 73        & 73     & 73 &\cellcolor[HTML]{969696} 7  &\cellcolor[HTML]{969696} 15  & \cellcolor[HTML]{969696}0   &\cellcolor[HTML]{969696} 0  \\
                             & non-matched & 39    & 0.44  & \cellcolor[HTML]{969696}87  &\cellcolor[HTML]{969696} 81        &\cellcolor[HTML]{969696} 93    & \cellcolor[HTML]{969696}87 & 20   & 99   & 87  & 92 \\ \hline
\end{tabular}
\label{tab:PSM-subgroup}
\end{table*}
